Long-Range Modeling of Source Code Files with eWASH: Extended Window Access by Syntax Hierarchy

Statistical language modeling and translation with transformers have found many successful applications in program understanding and generation tasks, setting high benchmarks for tools in modern software development environments. The finite context window of these neural models means, however, that they will be unable to leverage the entire relevant context of large files and packages for any given task. While there are many efforts to extend the context window, we introduce an architecture-independent approach for leveraging the syntactic hierarchies of source code for incorporating entire file-level context into a fixed-length window. Using concrete syntax trees of each source file we extract syntactic hierarchies and integrate them into context window by selectively removing from view more specific, less relevant scopes for a given task. We evaluate this approach on code generation tasks and joint translation of natural language and source code in Python programming language, achieving a new state-of-the-art in code completion and summarization for Python in the CodeXGLUE benchmark. We also introduce new CodeXGLUE benchmarks for user-experience-motivated tasks: code completion with normalized literals, method body completion/code summarization conditioned on file-level context.

==> recyled.tex <==
\iffalse
\begin{table}[htb]
\centering
\begin{tabular}{lc} 
\toprule
\textbf{Model}   &  \textbf{Accuracy(\%)} \\
\midrule
%LSTM + BPE &  \\
Transformer & 74.49 \\
%GPT-2 &  \\
CodeGPT & 76.58 \\
CodeGPT-adapted & 76.59 \\
GPT-C & \textbf{89.35} \\	
\bottomrule
\end{tabular}
\caption{Evaluation results on the next-token prediction code completion task with normalized literals add to the CodeXGLUE benchmark. Model performance metrics are reported on test set.} 
\label{tab:eval_codecompletion_token}	
\end{table}
\fi


\iffalse
\textbf{Perplexity} metric is used to evaluate the quality of language model pretraining of GPT-C models. It is defined as:
\begin{equation*}
PPL=exp(-\sum_{i}^{T}P(x_i)logP(x_i)),\forall i\in 0...T
\end{equation*}
where $x_i$ is the ground truth label and $P(x_i)$ is the model. The perplexity metric measures how well a model fits the data. A model with lower perplexity assigns higher probabilities to the true target tokens, thus is expected to be more superior for prediction.

\textbf{ROUGE} (Recall-Oriented Understudy for Gisting Evaluation) is a set of metrics generally used to evaluate machine translation. In the code completion problem, we adopt its Longest Common Subsequence (ROUGE-L) variant, which takes into
account code structure similarity by identifying longest co-occurring n-grams.

Developers are usually willing to accept a code completion suggestion with small edits afterwards. Motivated by this observation, we adopt \textbf{Levenshtein similarity} to measure how many single character edits – including insertion, substitution, or deletion – does it take to transform one sequence of code tokens to the ground truth.

\textbf{ExactMatch@N metrics}~\cite{exactmatch} allows us to measure how well a model can perfectly infer developers' intents at different suggestion lengths, i.e., match any ground truth code as exact. For each code completion point, if the N tokens long Top-1 best suggestion returned by a model exactly matches the first N ground truth tokens at the recommendation point, we count it as a “hit”. ExactMatch@N measures the ratio of the total number of hits to the total number of completion points.
\fi

\iffalse
\begin{figure}
\begin{minted}[
    xleftmargin=5pt,
    escapeinside=||,
    fontsize=\footnotesize,
    highlightlines={
        \getrefnumber{l0},
        \getrefnumber{l1},
        \getrefnumber{l2},
        \getrefnumber{l3},
    }
]{py}
import os, six, re

def isString(path):
    # hidden implementation
    
def isPath(path):
    # hidden implementation
    
def matchPattern(name, pattern):|\label{l0}|
    # hidden implementation|\label{l1}|
    
def findFiles(path, pattern):|\label{l2}|
    if |\label{l3}||\colorbox{gray}{             }|
\end{minted}
\caption{
A Python file in the process of being edited. The gray region is where code should be completed by an auto-regressive language model. The context window of the language model is finite and can only fit the region highlighted. In this case the desired completion is to validate \mintinline{py}{path} by predicting \mintinline{py}{not isPath(path):}, but the finite context window prevents the model from leveraging knowledge of the definition of \mintinline{py}{isPath}. eWASH solves this problem by training XGPT-C on abstracted code where the lower-level scopes of method bodies for example is hidden, and higher level scopes like function signatures and import statements are prioritized.
}
\label{fig:completion}
\end{figure}
\fi
% talk about IDE constraints

\iffalse
\section {Representing Source Code Programs}

Various source code representations have been proposed in literature~\cite{allamanis2017learning,code2vec}, differing by computational complexity and representation power. [cite] are built around abstract syntax trees, leveraging syntactic structure by decomposing programs into a collection of paths , [cite] encodes programs as graphs, in which edges represent syntactic relationships as well as semantic relationships like data flow. Treating programming languages as natural languages and modeling programs by constructing code sequences through an in-order traversal of the terminal nodes of a concrete syntax tree has been shown to be successful for several software engineering tasks~\cite{gptc, tufano2020generating, feng2020codebert}. While limited in the representation capacity, the latter approach is computationally the fastest. 

Modern IDEs have hundreds of extensions running concurrently in the same session. This imposes tight constraints on the memory consumption and the computational footprint: consuming many hundreds of megabytes of RAM would be prohibitive for a single component. From that perspective, sequence based representations of code are faster during inference. TODO: this is why we choose this rather than e.g. abstract semantic graph. Explain how we add syntactic hierarchies back

TODO: This section talks in great detail about the extended context, the source parser tool + a plot 

Global-file level context includes import statements, and variables defined in file scope outside classes and functions. 
Class-level extended context includes class signatures, class docstrings and class members defined in constructor. For each class method, it includes method decorators, signatures, docstrings. 
Function-level extended context includes function decorators, signatures, and docstrings.


%\MICHELE{Just a first draft of the context. Please feel free to rewrite.}
Our code representation closely resembles the canonical way that code is written by developers: organically structured at different levels of granularities. 

Source code belonging to different programming languages is commonly structured in the following granularities:
\begin{itemize}
    \item \textit{File-level}: defines the entire source code file (such as a \texttt{.py} or \texttt{.scala}). Instructions at this level influence globally the entire code within the file. For example, package declarations and imports establish the namespace and how libraries and APIs can be invoked throughout the entire file. This represents crucial information for a code generation approach, which should conform to the way imports are defined (\eg \texttt{import numpy as np} informs on the available APIs as well as the way they should be invoked) and possibly leverage global variables.
    \item \textit{Class-level}: defines a cohesive entity with internal states and functional behavior. Class name and docstring inform about the high-level concept which is implemented, variables specify internal states, while class methods define the available functionalities and interactions with the object. This data is of paramount importance for a model that aims at generating code for a particular class.
    \item \textit{Function-level}: defines an operation or process. The function name and docstring provide a synopsis of the intended behavior of the function, its signature provides the API through which it can be invoked, and its body enlists the low-level instructions that define its behavior. Such data can inform a code generation model on the requirements that need to be met for a given target method, or possible auxiliary methods that can be invoked.
\end{itemize}

In our representation we select code snippets -- sequence of \textit{tokens} -- from the aforementioned granularities to build the input to our code generation model. While constructing this representation we face two opposing goals: (i) include as many tokens as possible, given their powerful expressiveness discussed above (ii) keep a concise representation that fits into GPU memory.

To manage this balance we devise a priority-based code representation approach that aims at maximizing the usage of a given token \textit{budget}, which serve as a memory constraint.

Given a target function $f$ for which we are building the representation, we begin by selecting the tokens according to these priority levels:

\begin{itemize}
    \item Level-0
\begin{itemize}
    \item \textit{f.info}: according to the task, it can be a combination of \textit{f.docstring}, \textit{f.signature}, \textit{f.body}.
    \item \textit{File.imports}
    \item \textit{File.globalVars}
\end{itemize}
    \item Level-1
    \begin{itemize}
        \item \textit{Class.signature}
        \item \textit{Class.docstring}
        \item \textit{Class.vars}
        \item \textit{Function.signature}
        \item \textit{Function.docstring}
    \end{itemize}
    \item Level-2
    \begin{itemize}
        \item \textit{Function.body}
    \end{itemize}
\end{itemize}

Tokens are selected until the budget limit has been reached or all the tokens in the source code files have been covered.

Once the tokens are selected, they are printed as a sequence of tokens following the order in which they originally appear in the source code. The result is a code representation that closely resembles the original textual representation.


Representing code similarly to their textual representation has several advantages: (i) low extraction overhead; (ii) facilitate semi-supervised pretraining; (iii) facilitate inference. 

Discuss example...


% ---------- Code Example ----------------% TODO reformat with figure
\iffalse
\begin{figure}
    \centering

\begin{minted}[xleftmargin=20pt,linenos,escapeinside=||]{py}
from mylibrary import ExampleBaseClass
rom torch.nn import TransformerEncoder, \
    TransformerEncoderLayer

GLOBAL_CONSTANT = 1024


class ExampleClass(ExampleBaseClass):
    '''Example class docstring'''

    # class constructor
    def __init__(self, args, encoder, decoder):
        super().__init__(encoder, decoder)
        self.args = args

    # method
    def forward(self, src_tokens, src_lengths):
        '''Example method docstring'''

        encoder_out = self.encoder(
                src_tokens, 
                src_lengths=src_lengths
            )
        return encoder_out


if __name__ == "__main__":
    # example driver code
    args = {"supports_align_args": True}
    encoder_layer = TransformerEncoderLayer(d_model=512, nhead=8)
    transformer_encoder = TransformerEncoder(encoder_layer, num_layers=6)
    myclass = ExampleClass(args, transformer_encoder)
\end{minted}
\caption{An example program that implements a class in the Python programming language. A program consists of the import statements and a global variable, class definition, and the driver code that contains instantiation of the class.}
\label{fig:a}
\end{figure}
\fi
\fi
